Explainable Deep Learning Algorithm for Distinguishing Incomplete Kawasaki Disease by Coronary Artery Lesions on Echocardiographic Imaging

Background and Objective: Incomplete Kawasaki disease (KD) has often been misdiagnosed due to a lack of the clinical manifestations of classic KD. However, it is associated with a markedly higher prevalence of coronary artery lesions. Identifying coronary artery lesions by echocardiography is important for the timely diagnosis of and favorable outcomes in KD. Moreover, similar to KD, coronavirus disease 2019, currently causing a worldwide pandemic, also manifests with fever; therefore, it is crucial at this moment that KD should be distinguished clearly among the febrile diseases in children. In this study, we aimed to validate a deep learning algorithm for classification of KD and other acute febrile diseases. Methods: We obtained coronary artery images by echocardiography of children (n = 88 for KD; n = 65 for pneumonia). We trained six deep learning networks (VGG19, Xception, ResNet50, ResNext50, SE-ResNet50, and SE-ResNext50) using the collected data. Results: SE-ResNext50 showed the best performance in terms of accuracy, specificity, and precision in the classification. SE-ResNext50 offered a precision of 76.35%, a sensitivity of 82.64%, and a specificity of 58.12%. Conclusions: The results of our study suggested that deep learning algorithms have similar performance to an experienced cardiologist in detecting coronary artery lesions to facilitate the diagnosis of KD.

==> abs.tex <==
\textbf{Background and Objective:} Incomplete Kawasaki disease (KD) has often been misdiagnosed due to a lack of the clinical manifestations of classic KD. However, it is associated with a markedly higher prevalence of coronary artery lesions. Identifying coronary artery lesions by echocardiography is important for the timely diagnosis of and favorable outcomes in KD. Moreover, similar to KD, coronavirus disease 2019, currently causing a worldwide pandemic, also manifests with fever; therefore, it is crucial at this moment that KD should be distinguished clearly among the febrile diseases in children. In this study, we aimed to validate a deep learning algorithm for classification of KD and other acute febrile diseases. 

The incomplete Kawasaki disease (KD) has been often problematic to be misdiagnosed due to lack of the clinical manifestations of classic KD, but revealed with much higher prevalence of coronary artery lesion. 
Identifying coronary artery lesion by echocardiography is significant for the timely diagnosis and favorable outcome for KD. 
Moreover, the worldwide pandemic COVID-19 seems to be similar to KD in clinical manifestation with fever, therefore, it is very crucial moment that KD should be well detected between the febrile diseases in children. 
In this study, we validate the deep learning algorithm to classify KD and the other acute febrile disease. We obtained coronary artery images by echocardiography of children with 88 of KD and 65 of pneumonia. 
We trained six deep learning networks (VGG19, Xception, ResNet50, ResNext50, SE-ResNet50, and SE-ResNext50) using the collected data and the SE-ResNext50 offered a sensitivity of 82.64\% and a specificity of 58.12\%. 
The result of our study suggested that deep learning algorithms have similar performance to an experienced cardiologist for detecting the coronary artery lesion to help the diagnosis of KD.
